ABACuS: All-Bank Activation Counters for Scalable and Low Overhead RowHammer Mitigation

We introduce ABACuS, a new low-cost hardware-counter-based RowHammer mitigation technique that performance-, energy-, and area-efficiently scales with worsening RowHammer vulnerability. We observe that both benign workloads and RowHammer attacks tend to access DRAM rows with the same row address in multiple DRAM banks at around the same time. Based on this observation, ABACuS's key idea is to use a single shared row activation counter to track activations to the rows with the same row address in all DRAM banks. Unlike state-of-the-art RowHammer mitigation mechanisms that implement a separate row activation counter for each DRAM bank, ABACuS implements fewer counters (e.g., only one) to track an equal number of aggressor rows. Our evaluations show that ABACuS securely prevents RowHammer bitflips at low performance/energy overhead and low area cost. We compare ABACuS to four state-of-the-art mitigation mechanisms. At a near-future RowHammer threshold of 1000, ABACuS incurs only 0.58% (0.77%) performance and 1.66% (2.12%) DRAM energy overheads, averaged across 62 single-core (8-core) workloads, requiring only 9.47 KiB of storage per DRAM rank. At the RowHammer threshold of 1000, the best prior low-area-cost mitigation mechanism incurs 1.80% higher average performance overhead than ABACuS, while ABACuS requires 2.50X smaller chip area to implement. At a future RowHammer threshold of 125, ABACuS performs very similarly to (within 0.38% of the performance of) the best prior performance- and energy-efficient RowHammer mitigation mechanism while requiring 22.72X smaller chip area. ABACuS is freely and openly available at https://github.com/CMU-SAFARI/ABACuS.

==> sections/revision.tex <==

%\nobalance 
%\section*{{\Large AUTHORS' RESPONSE and SUMMARY OF CHANGES}}

% We thank the reviewers for their valuable feedback. We have addressed all comments. We first list the major changes we made to the paper in this revision. Then, we respond to each reviewer's comments and discuss how we have addressed them in the paper.  \\

\begin{center}
    \LARGE{\textbf{USENIX 2023 Revision for:}}\\
    \LARGE{\textit{ABACuS: All-Bank Activation Counters\\ for Scalable and Low Overhead RowHammer Mitigation}}
\end{center}

\vspace{10pt}

We thank the reviewers for their valuable feedback. We are addressing all Shepherd comments. We first list the major changes we made to the paper in this revision. Then, we respond to each Shepherd comment and discuss how we have addressed them in the paper.

The silver boxes list reviewer comments. We append our response for reviewer comments immediately below silver boxes. The yellow text box shows the changes made in the paper to address those comments. We use \textcolor{goodgreen}{green}, \textcolor{red}{red}, \reviii{purple}, and \revv{orange} to highlight the changes made to address \textcolor{goodgreen}{Comment 1}, \textcolor{red}{Comment 2}, \reviii{Comment 3}, and \revv{Comment 5}. We use the color \textcolor{blue}{blue} to highlight changes we made to address common concerns and improve the clarity in different sections in the paper.\\


MAJOR CHANGES TO THE PAPER:
\begin{enumerate}
	\item We revised \secref{sec:introduction} (\emph{``Introduction''}) and \secref{sec:motivation} (\emph{``Motivation''}) to highlight that RowHammer attacks can repeatedly access multiple sibling rows at around the same time, especially with the prefetch requests generated by simple prefetchers. This addresses Shepherd Comment 1.
 
	\item We revised \secref{sec:motivation} (\emph{``Motivation''}) to clarify our motivational analysis methodology and test with different window sizes. This addresses Shepherd Comment 2.

    \item We added performance and DRAM energy results for another random access workload, Giga Updates Per Second (GUPS) in \secref{sec:evaluation} (\emph{``Evaluation Methodology''}). We evaluated \X{} and prior work with carefully-engineered RowHammer access pattern that exacerbate \X{} and Hydra's performance overheads in \secref{sec:performance-under-attack} (\emph{``Performance Under RowHammer Attacks''}). We describe and evaluate a different \X{} version that performs well under such carefully-engineered access patterns in \secref{sec:abacus-big} (\emph{``Improving \X{}'s Performance Under RowHammer Attacks''}). This addresses Shepherd Comment 3.

    \item We expand on the ``RowHammer Mitigation in Commodity Chips'' discussion in \secref{sec:related} (\emph{``Related Work''}) by describing 1)~the performance overheads of commodity target row refresh (TRR) mechanisms and 2)~an analysis of the RowHammer threshold values that such mechanisms and their enhanced versions can securely prevent RowHammer bitflips at. This addresses Shepherd Comment 5.

    \item We 1)~moved three parts of the main text to the Appendix and 2)~drew compact versions of \figref{fig:perf_single_core_small} and \figref{fig:energy_single_core_small} to fit the paper into the page limit. We modified text to keep the paper self-contained and make the paper more compact. We highlighted all text modifications using \revcommon{blue} color. We list the components of the paper that we have moved to the Appendix: 
    \begin{itemize}
        \item Algorithm~\ref{algorithm:mech} to Appendix~\ref{appendix:algorithm} (previously in \secref{sec:mechanism-operation}).
        \item Detailed security analysis to Appendix~\ref{appendix:security-proof} (previously in \secref{sec:security-analysis}).
        \item Per-workload single-core performance and energy result plots and multi-core performance and energy results (previously in \secref{sec:evaluation-performance-energy}) to Appendices \secref{appendix:single-core-extended} and \secref{appendix:multi-core}.
    \end{itemize}
    % First, we moved Algorithm~\ref{algorithm:mech} to Appendix~\ref{appendix:algorithm} (previously in Section~\ref{sec:mechanism-operation}) and made the text in Section~\ref{sec:mechanism-operation} that previously relied on Algorithm~\ref{algorithm:mech} self contained. Second, we moved the detailed security analysis to Appendix~\ref{appendix:security-proof} (previously in Section~\ref{sec:security-analysis}) and modified Section~\ref{sec:security-analysis} to give a high-level overview of the security analysis. Third, we moved the per-workload single-core performance and energy result plots and multi-core performance and energy results (previously in Section~\ref{sec:evaluation-performance-energy}) to Appendices~\ref{appendix:single-core-extended} and Appendices~\ref{appendix:multi-core}, respectively.

	\item We revised the writing in multiple different sections to make our arguments and descriptions more clear. We use the color \textcolor{blue}{blue} to highlight these changes.
\end{enumerate}

%We respond to each reviewer's feedback in detail on the following pages, and describe the associated changes we made to the revised paper, including changes based on all other comments.

% \renewcommand\contentsname{} % the empty name
% \vspace{5pt}
% \setcounter{tocdepth}{-1}

% \tableofcontents 
% \addtocontents{toc}{~\hfill\textbf{Page}\par}

% \tableofcontents
\def\mydots{\leavevmode\xleaders\hbox to 0.45em{\hfil.\hfil}\hfill\kern0pt}

\vspace{25pt}



\noindent \textbf{\large{Contents}} 
\vspace{5pt}

\noindent \textbf{\hyperlink{comment1}{Comment 1}}~\mydots~~26
\vspace{5pt}

\noindent \textbf{\hyperlink{comment2}{Comment 2}}~\mydots~~27
\vspace{5pt}

\noindent \textbf{\hyperlink{comment3}{Comment 3}}~\mydots~~30
\vspace{5pt}

\noindent \textbf{\hyperlink{comment5}{Comment 5}}~\mydots~~33
\vspace{5pt}

\newpage
%\section*{{\Large \normalfont{\textbf{REVIEWER 1}}}}
\begin{center}
    {\Large \normalfont{\textbf{\hypertarget{comment1}{Comment 1}}}}
\end{center}

\begin{tcolorbox}
    \begin{enumerate}[label=C\arabic*)]
        \item \label{c:c1} Evaluate the bank/row locality of different RowHammer strategies.
    \end{enumerate}
\end{tcolorbox} 

We thoroughly investigate recent RowHammer attacks and identify two commonly-used strategies: i) double-sided (e.g., in~\cite{kim2020revisiting,orosa2021deeper,seaborn2015exploiting,pessl2016drama,razavi2016flip,jang2017sgx,tatar2018defeating}) and ii) many-sided (e.g., in~\cite{deridder2021smash,hassan2021utrr,frigo2020trrespass,cohen2022hammerscope,jattke2022blacksmith,kogler2022half}) RowHammer attacks. We craft memory traces that represent these two strategies combined with different configurations of a simple prefetching mechanism in the system to understand these strategies' bank/row locality.

\setcounter{figure}{1}
\vspace{5pt}
\yyboxbegin
\Paste{C1}
\begin{center}
\begin{minipage}{1.0\linewidth}
   \captionsetup{type=figure} % -- added
   \Paste{C1fig}
\end{minipage}
\end{center}
\yyboxend

We revise the introduction to include RowHammer attacks as part of \X{}'s motivation.

\vspace{5pt}
\yyboxbegin
\Paste{C1intro}
\yyboxend

\newpage
\begin{center}
    {\Large \normalfont{\textbf{\hypertarget{comment2}{Comment 2}}}}
\end{center}

\begin{tcolorbox}
    \begin{enumerate}[label=C\arabic*)]
        \addtocounter{enumi}{1}
        \item \label{c:c2} Evaluate different window sizes.
    \end{enumerate}
\end{tcolorbox} 

We revise our motivational analysis methodology to clarify how we motivate why we use row activation counters shared across sibling rows. Instead of showing how many sibling rows are activated in a fixed size of activation windows (i.e., continuous set of \act{} commands), our revision shows the number of times a sibling row gets activated (i.e., receives an \act{} command) \emph{when} an aggressor sibling row is activated \gls{nrh} times. The key idea is that a higher sibling row activation count indicates that the aggressor sibling row's activation count can be used to accurately track the activation counts of all siblings of the aggressor row. We plot three different graphs with three different \gls{nrh} values to show how the activation counts of sibling rows change with \gls{nrh}.

All of our changes are in \secref{sec:motivation} (\emph{``Motivation''}).

\setcounter{figure}{1}

\vspace{5pt}
\yyboxbegin
\Paste{C2/1}
\Paste{C2/2}
\begin{center}
\begin{minipage}{1.0\linewidth}
   \captionsetup{type=figure} % -- added
   \Paste{C1fig}
\end{minipage}
\end{center}
\yyboxend

\newpage
\yyboxbegin
\Paste{C2/3}

\Paste{C2/4}

\begin{center}
\begin{minipage}{0.6\linewidth}
   \captionsetup{type=figure} % -- added
   \Paste{C2fig}
\end{minipage}
\end{center}
\newline
\newpage
\Paste{C2/5}
\yyboxend

\newpage

\begin{center}
    {\Large \normalfont{\textbf{\hypertarget{comment3}{Comment 3}}}}
\end{center}


\begin{tcolorbox}
    \begin{enumerate}[label=C\arabic*)]
        \addtocounter{enumi}{2}
        \item \label{c:c3} Evaluate ABACuS with worst case workloads, most likely random-access workloads.
    \end{enumerate}
\end{tcolorbox} 

We include the ``Giga Updates per Second (GUPS)'' workload (as suggested by Reviewer E) in our evaluation of \X{}'s performance and energy efficiency in addition to multiple random-access workloads (e.g., 429.mcf and 470.lbm) that we evaluated in our submission. 

The revised version adds the results for the gups workload to all relevant figures in Sections~\ref{sec:evaluation-performance-energy} and~\ref{sec:motivation} (omitted from our revision summary for brevity).

We added footnote 3 to Section~\ref{sec:motivation}.

\vspace{5pt}
\yyboxbegin
\Paste{C3f1}
\yyboxend

\setcounter{table}{3}
We updated Table~\ref{table:workloads}.

\vspace{5pt}
\yyboxbegin
\begin{center}
\begin{minipage}{0.6\linewidth}
   \captionsetup{type=table} % -- added
   \Paste{C3table}
\end{minipage}
\end{center}
\yyboxend


We updated text describing key results and all performance/energy evaluation numbers that we report throughout the paper (we omit these numbers from our revision summary to keep the summary compact).

%Revised Figures~\ref{fig:perf_single_core}-\ref{fig:energy_comparison_multi_core} in Section~\ref{sec:evaluation-performance-energy} include the results for the GUPS workload. 
%fig:perf_comparison_multi_core,fig:energy_comparison_multi_core,fig:perf_single_core,fig:energy_single_core} with new results.

\newpage

A motivated attacker who is aware of the existence of \X{} in the system can develop workloads with specialized access patterns that aim to exacerbate \X{}'s performance overheads. We expand Section~\ref{sec:performance-under-attack} where we analyze the performance of prior mitigation techniques and \X{} when these techniques are subject to worst-case access patterns. Revised Section~\ref{sec:performance-under-attack} describes the hand-crafted access patterns and our results in more detail.

\setcounter{figure}{11}
\vspace{5pt}
\yyboxbegin
\Paste{C3/2}
\begin{center}
\begin{minipage}{0.6\linewidth}
   \captionsetup{type=figure} % -- added
   \Paste{C3fig}
\end{minipage}
\end{center}
\Paste{C3/3}
\yyboxend

\newpage

We develop and evaluate an alternative \X{} design which is \emph{not} subject to performance degradation under RowHammer attacks. Revised Section~\ref{sec:performance-under-attack} describes this new design and discusses the results of our evaluation.

\vspace{5pt}
\yyboxbegin
\Paste{C3/4}
\begin{center}
\begin{minipage}{0.6\linewidth}
   \captionsetup{type=figure} % -- added
   \Paste{C3fig2}
\end{minipage}
\end{center}
\Paste{C3/5}
\yyboxend

\newpage

\begin{center}
    {\Large \normalfont{\textbf{\hypertarget{comment5}{Comment 5}}}}
\end{center}


\begin{tcolorbox}
    \begin{enumerate}[label=C\arabic*)]
        \addtocounter{enumi}{4}
        \item \label{c:c5} Include a ``schoolbook'' TRR implementation (using reverse-engineered data e.g., from TRRespass such as the number of counters, and reasonable threshold choices) in the evaluations.
    \end{enumerate}
\end{tcolorbox} 

Known Target Row Refresh (TRR) implementations on commercial DRAM chips do \emph{not} induce performance overheads. We acknowledge this in the revision and present a detailed security evaluation of a widespread TRR implementation in \secref{sec:related} to show that this TRR implementation cannot prevent RowHammer bitflips at today's or future RowHammer thresholds. 

\vspace{5pt}
\yyboxbegin
\Paste{C5/1}

\Paste{C5/2}
\begin{center}
\begin{minipage}{0.6\linewidth}
   \captionsetup{type=figure} % -- added
   \Paste{C5fig}
\end{minipage}
\end{center}

\Paste{C5/3}
\yyboxend

